Network Capacity Bound for Personalized PageRank in Multimodal Networks

In a former paper the concept of Bipartite PageRank was introduced and a theorem on the limit of authority flowing between nodes for personalized PageRank has been generalized. In this paper we want to extend those results to multimodal networks. In particular we deal with a hypergraph type that may be used for describing multimodal network where a hyperlink connects nodes from each of the modalities. We introduce a generalisation of PageRank for such graphs and define the respective random walk model that can be used for computations. We state and prove theorems on the limit of outflow of authority for cases where individual modalities have identical and distinct damping factors.

==> macro.tex <==
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{url}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\newcommand{\keywords}[1]{\quad \\ {\bf Keywords: }{\it #1} }
\newcommand{\rys}[1]{}
\newcommand{\citep}{\cite}
\newcommand{\wyrzucicv}[1]{\textbf{}}

\newcommand{\fan}{enthusiast}

\newcommand{\Bem}[1]{}
\newcommand{\HEM}{\mathcal{E}}
% single hyper edge multimodal
\newcommand{\hem}{\mathfrak{e}}
% hypergraph multimodal
\newcommand{\HGM}{\mathcal{H}}
% set of nodes
\newcommand{\N}{ V }
% a node
\newcommand{\n}{ v }
% plain hyperedger
\newcommand{\h}{e}
% plain hypergraph
\newcommand{\HG}{H}
% plain set of hyperedges
\newcommand{\HE}{E}
% generalized graph
\newcommand{\GG}{\mathcal{G}}
% generalized edge set
\newcommand{\GE}{\mathbf{E}}
% generalized edge
\newcommand{\Ge}{\mathbf{e}}
% generalized node set
\newcommand{\GN}{\mathbf{V}}

\newcommand{\Zeta}{\boldsymbol\zeta}





%\begin{document}
%\input teskZglvoszonyWPazxdzierniku
\input MuMoRank_maj2023

%\input uwagiRecenzentaMaj2023
%\input responsestothereviewers

